From data to reduced-order models via moment matching

A new method for data-driven interpolatory model reduction is presented in this paper. Using the so-called data informativity perspective, we define a framework that enables the computation of moments at given (possibly complex) interpolation points based on time-domain input-output data only, without explicitly identifying the high-order system. Instead, by characterizing the set of all systems explaining the data, necessary and sufficient conditions are provided under which all systems in this set share the same moment at a given interpolation point. Moreover, these conditions allow for explicitly computing these moments. Reduced-order models are then derived by employing a variation of the classical rational interpolation method. The condition to enforce moment matching model reduction with prescribed poles is also discussed as a means to obtain stable reduced-order models. An example of an electrical circuit illustrates this framework.

==> myfigureUY.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=2.73in,
height=2.1in,
at={(0.898in,0.499in)},
scale only axis,
xmin=0,
xmax=4,
xlabel style={font=\color{white!15!black}},
xlabel={Time},
ymin=-4,
ymax=6,
ylabel style={font=\color{white!15!black}},
ylabel={Input and Output},
axis background/.style={fill=white},
legend style={at={(0.705,0.805)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot[const plot, color=mycolor1, line width=1.2pt] table[row sep=crcr] {%
0	6\\
0.2	4.82842712474619\\
0.4	1.5\\
0.6	-1.82842712474619\\
0.8	-3.375\\
1	-2.45342712474619\\
1.2	0.218750000000001\\
1.4	2.95342712474619\\
1.6	4.0703125\\
1.8	2.86748962474619\\
2	0.0214843749999994\\
2.2	-2.81670837474619\\
2.4	-3.99365234375\\
2.6	-2.82500915599619\\
2.8	0.00183105468750065\\
3	2.82940368724619\\
3.2	4.00051879882812\\
3.4	2.82870178294931\\
3.6	0.000144958496092528\\
3.8	-2.82835083080087\\
4	-3.9999599456787\\
};
\addlegendentry{Input}

\addplot[const plot, color=mycolor2, dashdotted, line width=1.2pt] table[row sep=crcr] {%
0	0\\
0.2	0.750142693163355\\
0.4	1.08116685317361\\
0.6	0.980491187502263\\
0.8	0.595913339752955\\
1	0.191902330870994\\
1.2	0.0157380976962526\\
1.4	0.166785174526049\\
1.6	0.546122055875743\\
1.8	0.91843947113271\\
2	1.05175659783095\\
2.2	0.854155765536378\\
2.4	0.427981299765709\\
2.6	0.0100198261318992\\
2.8	-0.167171061483162\\
3	-0.0114970163140711\\
3.2	0.374705095292879\\
3.4	0.754589665342779\\
3.6	0.89551762108953\\
3.8	0.705308450373642\\
4	0.286214797497349\\
};
\addlegendentry{Output}

\end{axis}
\end{tikzpicture}%

==> table.tex <==
\begin{tabular}{|r|r|r||r|r|r|}
			\hline
			$t$ & $U$ & $Y$ & $t$ & $U$ & $Y$ \\
			\hline
			$0$ &  $ 2$   &    $ 0 $ & $11  $ & $ -0.7012  $ & $  0.3108$
			\\
			$1$ & $ 1.7071$ & $0.25$ & $12  $ & $ -0.9968  $ & $  0.1996$
			\\
			$2  $ & $  0.7500  $ & $  0.3726$  & $13  $ & $ -0.7054  $ & $ 0.0907$
			\\
			$3  $ & $ -0.2071  $ & $  0.3659$ & $14  $ & $  0.0009 $ & $   0.0422$
			\\
			$4  $ & $ -0.6875  $ & $  0.2755$ & $15  $ & $  0.7076 $ & $   0.0772$
			\\
			$5  $ & $ -0.5196  $ & $  0.1738$ & $16  $ & $  1.0003  $ & $  0.1699$
			\\
			$6  $ & $  0.1094  $ & $  0.1262$ & $17  $ & $  0.7072 $ & $   0.2613$
			\\
			$7   $ & $ 0.7696  $ & $  0.1592$ & $18  $ & $  0.0001  $ & $  0.2931$
			\\
			$8 $ & $  1.0352 $ & $  0.2488$ & $19 $ & $  -0.7071 $ & $   0.2422$
			\\
			$9  $ & $  0.7266  $ & $  0.3367$ & $20 $ & $  -1  $ & $  0.1343 $
			\\
			$10  $ & $  0.0107 $ & $   0.365$ & & & 
			\\
			\hline
		\end{tabular}
